A Flexible Model for Record Linkage

Combining data from various sources empowers researchers to explore innovative questions, for example those raised by conducting healthcare monitoring studies. However, the lack of a unique identifier often poses challenges. Record linkage procedures determine whether pairs of observations collected on different occasions belong to the same individual using partially identifying variables (e.g. birth year, postal code). Existing methodologies typically involve a compromise between computational efficiency and accuracy. Traditional approaches simplify this task by condensing information, yet they neglect dependencies among linkage decisions and disregard the one-to-one relationship required to establish coherent links. Modern approaches offer a comprehensive representation of the data generation process, at the expense of computational overhead and reduced flexibility. We propose a flexible method, that adapts to varying data complexities, addressing registration errors and accommodating changes of the identifying information over time. Our approach balances accuracy and scalability, estimating the linkage using a Stochastic Expectation Maximisation algorithm on a latent variable model. We illustrate the ability of our methodology to connect observations using large real data applications and demonstrate the robustness of our model to the linking variables quality in a simulation study. The proposed algorithm FlexRL is implemented and available in an open source R package.

==> Figures/Fig3_phi/graphical_cv_phi.tex <==
\begin{figure}[!h]
    \centering
    \begin{tikzpicture}
    \node at (0.3,-1.2) {\textit{FlexRL} all stable};
    \node at (7.8,-1.2) {\textit{FlexRL} with instability};
    \node at (0,-3.5) {\scalebox{0.7}{\input{Figures/Fig3 phi/phi V1 stable}}};
    \node at (1.5,-2.4) {$1^{\text{st}}$ PIV};
    \node at (0,-7.35) {\scalebox{0.7}{\input{Figures/Fig3 phi/phi V5 stable}}};
    \node at (1.5,-6.24) {$5^{\text{th}}$ PIV};
    \node at (7.5,-3.5) {\scalebox{0.7}{\input{Figures/Fig3 phi/phi V1 instability}}};
    \node at (9,-2.4) {$1^{\text{st}}$ PIV};
    \node at (7.5,-7.35) {\scalebox{0.7}{\input{Figures/Fig3 phi/phi V5 instability}}};
    \node at (9,-6.24) {$5^{\text{th}}$ PIV};
    \node[rotate=90] at (-3.4,-5.425) {$\boldsymbol{\phi}_{\text{mistake}}$};
    \node[rotate=90] at (11.6,-5.425) {};
    \node at (4.1,-9.8) {StEM iterations};
    \end{tikzpicture}
    \caption{Probability of mistake represented by the parameter $\boldsymbol{\phi}_{\text{mistake}}$ for a stable PIV (here the $1^{\text{st}}$ one) and the unstable $5^{\text{th}}$ PIV. On the right is \textit{FlexRL} taking into account the instability of the $5^{\text{th}}$ PIV (in which case $\boldsymbol{\phi}_{\text{mistake}}$ is known and set to 0). On the left is \textit{FlexRL} considering all PIVs stable. The dotted thick line is the true probability. The solid thin line is the averaged estimated probability over the 500 simulations and the faded interval around corresponds to the estimated probability standard deviation, showing the simulations noise. We use the 25 last values of the parameter to build the final estimate of the linkage (we discard 75 iterations as burn-in).}
    \label{fig: graph_cv_param_phi}
\end{figure}


==> Figures/Fig4_gamma/graphical_cv_gamma.tex <==
\begin{figure}[!h]
    \centering
    \begin{tikzpicture}
    \node at (0.3,-5.55) {\textit{FlexRL} all stable};
    \node at (7.8,-5.55) {\textit{FlexRL} with instability};
    \node at (0,-7.85) {\scalebox{0.7}{\input{Figures/Fig4 gamma/gamma stable}}};
    \node at (7.5,-7.85) {\scalebox{0.7}{\input{Figures/Fig4 gamma/gamma instability}}};
    \node at (-3.4,-7.85) {$\gamma$};
    \node at (11.6,-7.85) {};
    \node at (4.1,-10.3) {StEM iterations};
    \end{tikzpicture}
    \caption{Probability for a record in $\mathcal{A}$ to form a link with a record in $\mathcal{B}$ represented by the parameter $\gamma$. On the right is \textit{FlexRL} taking into account the instability of the $5^{\text{th}}$ PIV and on the left is \textit{FlexRL} considering all PIVs stable. The dotted thick line is the true proportion of links (as a fraction of the smallest file $\mathcal{A}$). The solid thin line is the averaged estimated probability over the 500 simulations and the faded interval around corresponds to the estimated probability standard deviation, showing the simulations noise. We use the 25 last values of the parameter to build the final estimate of the linkage (we discard 75 iterations as burn-in).}
    \label{fig: graph_cv_param_gamma}
\end{figure}


==> Figures/Fig7_FDR_Sensitivity_NLTCS/Fdr_Sensitivity.tex <==
\begin{figure}[!h]
    \centering
    \begin{tikzpicture}
    \pgfplotsset{
    width=0.5\textwidth,
    height=0.3\textwidth}
    \begin{axis}[
        xmin=0, xmax=1,
        ymin=0, ymax=1,
        xtick={0,0.2,0.4,0.6,0.8,1},
        ytick={0,0.2,0.4,0.6,0.8,1},
        xlabel={Sensitivity},
        ylabel={FDR}
        ]
        % Simplistic for all scenarios:
    \node[minimum size=1mm, inner sep=4pt, draw, rectangle] (simplistic_state_reg) at (0.88, 0.65) {};
        % FlexRL: scenario: state and region
    \addplot[smooth, dotted, thick] plot coordinates { 
        (0.4269574, 0.4869771)
        (0.3775617, 0.4342520)
        (0.3384130, 0.3887043)
        (0.3030741, 0.3481209)
        (0.2673410, 0.3064076) };
    \node[minimum size=1mm, inner sep=1.5pt, draw, circle, thick, dotted, fill=white] (FlexRLdefault_state_reg) at (0.426957435627956, 0.486977111286504) {};
    \node[minimum size=0.7mm, inner sep=0.7pt, draw, star, star points=7,star point ratio=0.3, fill=white] (FlexRLcontrolled_state_reg) at (0.36, 0.41) {};
        % FlexRL: scenario: state and region glued / state only
    \addplot[smooth] plot coordinates { 
        (0.21647406611126, 0.109452736318408)
        (0.1845770, 0.1016624)
        (0.1382028, 0.08759757)
        (0.09774041, 0.07347447)
        (0.05977404, 0.05601660)
        (0.01523910, 0.05691057) };
    \node[minimum size=1mm, inner sep=1.5pt, draw, circle, fill=black] (FlexRLdefault_state) at (0.21647406611126, 0.109452736318408) {};
    \node[minimum size=0.7mm, inner sep=0.7pt, draw, star,star points=7,star point ratio=0.3, fill=black] (FlexRLcontrolled_state) at (0.04, 0.056) {};
    \end{axis}
\end{tikzpicture}
    \caption{Evolution of the FDR and the sensitivity for three scenarios: using the state and regional codes as PIVs (\textit{FlexRL} dotted line), merging those PIVs into one and considering the state code only (both represented for \textit{FlexRL} as a solid line). Each line represents the true FDR and true sensitivity obtained for different level of threshold $\xi \in [0.5 , 1]$ on the linkage probabilities to select a final set of linked records. Round symbols correspond to the metrics obtained for $\xi = 0.5$ and star symbols to the metrics obtained by controlling the estimated FDR to be lower than $10\%$. The square symbol represent the metrics obtained by the simplistic approach.}
    \label{fig: FDR Sensitivity NLTCS complete data}
\end{figure}



==> Figures/FigSuppl_Distortion/FlexRL_SHIW.tex <==
\begin{tikzpicture}[x=1pt,y=1pt]
    \begin{axis}[
        xmin=-0.05, xmax=0.45,
        ymin=0, ymax=1,
        xtick={0,0.1,0.2,0.3,0.4},
        ytick={0,0.2,0.4,0.6,0.8,1},
        legend style={at={(0.9,0.59)}},
        legend entries={F1-Score, FDR, Sensitivity} ]
    \addplot[smooth,dashed] plot coordinates { (0.04,0.31)
        (0.12,0.26)
        (0.19,0.22)
        (0.27,0.18)
        (0.34,0.16)
        (0.40,0.14) };
    \addplot[smooth] plot coordinates { (0.04,0.73)
        (0.12,0.76)
        (0.19,0.78)
        (0.27,0.80)
        (0.34,0.81)
        (0.40,0.82) };
    \addplot[smooth,dotted] plot coordinates { (0.04,0.38)
        (0.12,0.28)
        (0.19,0.23)
        (0.27,0.17)
        (0.34,0.14)
        (0.40,0.11) };
    \end{axis}
\end{tikzpicture}

==> Figures/FigSuppl_Distortion/Simplistic_SHIW.tex <==
\begin{tikzpicture}[x=1pt,y=1pt]
    \begin{axis}[
        xmin=-0.05, xmax=0.45,
        ymin=0, ymax=1,
        xtick={0,0.1,0.2,0.3,0.4},
        ytick={0,0.2,0.4,0.6,0.8,1},
        legend style={at={(0.9,0.59)}},
        legend entries={F1-Score, FDR, Sensitivity} ]
    \addplot[smooth,dashed] plot coordinates { (0.04,0.35)
        (0.12,0.30)
        (0.19,0.25)
        (0.27,0.20)
        (0.34,0.16)
        (0.40,0.12) };
    \addplot[smooth] plot coordinates { (0.04,0.76)
        (0.12,0.78)
        (0.19,0.80)
        (0.27,0.83)
        (0.34,0.86)
        (0.40,0.88) };
    \addplot[smooth,dotted] plot coordinates { (0.04,0.67)
        (0.12,0.49)
        (0.19,0.35)
        (0.27,0.24)
        (0.34,0.18)
        (0.40,0.13) };
    \end{axis}
\end{tikzpicture}

==> Figures/FigSuppl_Distortion/perf_distortion_SHIW.tex <==
\begin{figure}[!h]
    \centering
    \begin{tikzpicture}
    \node at (0.3,-5.55) {\textit{FlexRL}};
    \node at (7.8,-5.55) {Simplistic};
    \node at (0,-7.85) {\scalebox{0.7}{\input{Figures/FigSuppl_Distortion/FlexRL_SHIW}}};
    \node at (7.5,-7.85) {\scalebox{0.7}{\input{Figures/FigSuppl_Distortion/Simplistic_SHIW}}};
    \node at (4.1,-10.3) {Distortion};
    \end{tikzpicture}
    \caption{Evolution of the F1-score, FDR and sensitivity for screwed versions of the complete SHIW data sets. We artificially distort the data and we define the distortion level (x-axis) as the sum of medians of disagreements and missing values among the PIVS of true links.}
    \label{fig_performancesXdeformationsSHIW}
\end{figure}

==> Figures/FigSuppl_Hist_Proba/histogram_linkage_proba.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        ymin=0, ymax=10,
        ytick={0,2,4,6,8,10},
        yticklabels={$\log_{10} 10^{0\hphantom{0}}$, $\log_{10} 10^{2\hphantom{0}}$, $\log_{10} 10^{4\hphantom{0}}$, $\log_{10} 10^{6\hphantom{0}}$, $\log_{10} 10^{8\hphantom{0}}$, $\log_{10} 10^{10}$} 
        ]
    \addplot+[ybar interval, mark=no, draw=black
    ] plot coordinates { (0, 8.39) (0.05, 3.80) (0.1, 3.64) (0.15, 3.50) (0.2, 3.39) (0.25, 3.30) (0.3, 3.19) (0.35, 3.10) (0.4, 3.02) (0.45, 2.96) (0.5, 2.89) (0.55, 2.83) (0.6, 2.75) (0.65, 2.73) (0.7, 2.66) (0.75, 2.67) (0.8, 2.64) (0.85, 2.62) (0.9, 2.68) (0.95, 3.64) (1, 3.64) };
    \end{axis}
    \end{tikzpicture}
    \caption{Linkage probabilities in \smash{$\boldsymbol{\hat\Delta}$} on a log (base 10) scale for the SHIW data sets. The bimodal distribution is representing the mixture between links and non links (and uncertain cases in between).}
    \label{fig_SHIWprobaDeltaHist}
\end{figure}

==> Figures/FigSuppl_Regional_Boxplots_SHIW/Boxplots_SHIW.tex <==
\begin{figure}[!h]
    \centering
    \begin{tikzpicture}
    \node at (0.3,-5.27) {F1-Score};
    \node at (5.8,-5.27) {False Discovery Rate};
    \node at (11.3,-5.27) {Sensitivity};
    \node at (0,-7.85) {\scalebox{0.7}{\input{Figures/FigSuppl_Regional_Boxplots_SHIW/F1Score_SHIW}}};
    \node at (5.5,-7.85) {\scalebox{0.7}{\input{Figures/FigSuppl_Regional_Boxplots_SHIW/FDR_SHIW}}};
    \node at (11,-7.85) {\scalebox{0.7}{\input{Figures/FigSuppl_Regional_Boxplots_SHIW/Sensitivity_SHIW}}};
    \end{tikzpicture}
    \caption{Boxplots showing the variability of the F1-score, the FDR and the sensitivity of the compared methods on regional subsets of the SHIW data sets: Piedmont, Aosta Valley, Lombardy, Trentino-Alto Adige, Veneto, Friuli–Venezia Giulia, Liguria, Emilia–Romagna, Tuscany, Umbria, Marche, Lazio, Abruzzo, Molise, Campania, Apulia, Basilicata, Calabria, Sicily, Sardinia.}
    \label{fig_Regional_Boxplots_SHIW}
\end{figure}

==> Figures/FigSuppl_Regional_Boxplots_SHIW/F1Score_SHIW.tex <==
\begin{tikzpicture}[x=1pt,y=1pt]
      \begin{axis}
        [
        boxplot/draw direction=y,
        ymin=0,ymax=1,
        % ylabel={F1 Score},
        xtick={1,2,3,4},
        xticklabels={\textit{FlexRL}, \textit{Exchanger}, \textit{BRL}, Simplistic},
        cycle list={{black},{black},{black},{black}}
        ]
        \addplot+[mark = o,
        boxplot prepared={
          lower whisker  =0.1775,
          lower quartile =0.3588,
          median         =0.3875,
          upper quartile =0.5544,
          upper whisker  =0.7826
        },
        ] coordinates {(0,0.3649123)(0,0.7826087)(0,0.3698469)(0,0.3585434)(0,0.2727273)(0,0.5629630)(0,0.5902778)(0,0.3591549)(0,0.3747981)(0,0.4587525)(0,0.5458613)(0,0.3800384)(0,0.4695652)(0,0.7567568)(0,0.2240326)(0,0.2282794)(0,0.6878307)(0,0.4744526)(0,0.1775148)(0,0.3949580)};
        \addplot+[mark = o,
        boxplot prepared={
          lower whisker  =0.0693,
          lower quartile =0.0955,
          median         =0.1607,
          upper quartile =0.2837,
          upper whisker  =0.4875
        },
        ] coordinates {(0,0.07858688)(0,0.57777780)(0,0.07016992)(0,0.10763640)(0,0.10509140)(0,0.25423730)(0,0.31319910)(0,0.09767092)(0,0.14671420)(0,0.19984740)(0,0.23725060)(0,0.11382110)(0,0.35409840)(0,0.48745520)(0,0.09333850)(0,0.06933020)(0,0.38805970)(0,0.22845690)(0,0.07900751)(0,0.17469390)};
        \addplot+[mark = o,
        boxplot prepared={
          lower whisker  =0.0771,
          lower quartile =0.1702,
          median         =0.3537,
          upper quartile =0.5200,
          upper whisker  =0.7692
        },
        ] coordinates {(0,0.20309051)(0,0.76923077)(0,0.10603829)(0,0.34626866)(0,0.16532258)(0,0.56716418)(0,0.57358491)(0,0.17500000)(0,0.29811321)(0,0.45575221)(0,0.46650124)(0,0.28633406)(0,0.41121495)(0,0.69444444)(0,0.14562002)(0,0.14772727)(0,0.67692308)(0,0.47286822)(0,0.07709751)(0,0.36117381)};
        \addplot+[mark = o,
        boxplot prepared={
          lower whisker  =0.2467,
          lower quartile =0.3368,
          median         =0.4350,
          upper quartile =0.5505,
          upper whisker  =0.7826
        },
        ] coordinates {(0,0.3562264)(0,0.7826087)(0,0.2866044)(0,0.4327323)(0,0.3392659)(0,0.5944444)(0,0.5737705)(0,0.3342906)(0,0.3840304)(0,0.4867359)(0,0.527227)(0,0.3937138)(0,0.5111111)(0,0.6533865)(0,0.2625087)(0,0.2930944)(0,0.6439024)(0,0.5132743)(0,0.2467357)(0,0.4372256)};
      \end{axis}
      % \node[above,font=\bfseries] at (current bounding box.north) {F1 Score};
      \end{tikzpicture}

==> Figures/FigSuppl_Regional_Boxplots_SHIW/FDR_SHIW.tex <==
\begin{tikzpicture}[x=1pt,y=1pt]
      \begin{axis}
        [
        boxplot/draw direction=y,
        ymin=0,ymax=1,
        % ylabel={FDR},
        xtick={1,2,3,4},
        xticklabels={\textit{FlexRL}, \textit{Exchanger}, \textit{BRL}, Simplistic},
        cycle list={{black},{black},{black},{black}}
        ]
        \addplot+[mark = o,
        boxplot prepared={
          lower whisker  =0.1818,
          lower quartile =0.2806,
          median         =0.3486,
          upper quartile =0.4176,
          upper whisker  =0.5161
        },
        ] coordinates {(0,0.4285714)(0,0.1818182)(0,0.2629108)(0,0.3786408)(0,0.3809524)(0,0.2830189)(0,0.3200000)(0,0.3245033)(0,0.4423077)(0,0.3736264)(0,0.2781065)(0,0.3028169)(0,0.4065934)(0,0.1923077)(0,0.4472362)(0,0.4508197)(0,0.2441860)(0,0.3500000)(0,0.5161290)(0,0.3472222)};
        \addplot+[mark = o,
        boxplot prepared={
          lower whisker  =0.5776,
          lower quartile =0.7887,
          median         =0.8937,
          upper quartile =0.9435,
          upper whisker  =0.9610
        },
        ] coordinates {(0,0.9543168)(0,0.3809524)(0,0.9610140)(0,0.9339875)(0,0.9385027)(0,0.8239437)(0,0.7535211)(0,0.9420935)(0,0.9072165)(0,0.8683417)(0,0.8285256)(0,0.9327247)(0,0.6746988)(0,0.5776398)(0,0.9449772)(0,0.9598503)(0,0.6020408)(0,0.8246154)(0,0.9543224)(0,0.8801792)};
        \addplot+[mark = o,
        boxplot prepared={
          lower whisker  =0.1628,
          lower quartile =0.2453,
          median         =0.2809,
          upper quartile =0.3298,
          upper whisker  =0.4133
        },
        ] coordinates {(0,0.2923077)(0,0.2857143)(0,0.1627907)(0,0.2839506)(0,0.1800000)(0,0.2692308)(0,0.2549020)(0,0.3333333)(0,0.3361345)(0,0.2426471)(0,0.2480000)(0,0.1951220)(0,0.4133333)(0,0.2346939)(0,0.3263158)(0,0.3809524)(0,0.2826087)(0,0.2738095)(0,0.3703704)(0,0.2792793)};
        \addplot+[mark = o,
        boxplot prepared={
          lower whisker  =0.1818,
          lower quartile =0.5327,
          median         =0.6787,
          upper quartile =0.7773,
          upper whisker  =0.8484
        },
        ] coordinates {(0,0.7481323)(0,0.1818182)(0,0.8162450)(0,0.6659529)(0,0.7744083)(0,0.4540816)(0,0.4827586)(0,0.7802115)(0,0.7403599)(0,0.6170599)(0,0.5981132)(0,0.7132530)(0,0.5837104)(0,0.3834586)(0,0.8394535)(0,0.8058659)(0,0.3529412)(0,0.5827338)(0,0.8483675)(0,0.6914498)};
      \end{axis}
      % \node[above,font=\bfseries] at (current bounding box.north) {False Discovery Rate};
      \end{tikzpicture}

==> Figures/FigSuppl_Regional_Boxplots_SHIW/Sensitivity_SHIW.tex <==
\begin{tikzpicture}[x=1pt,y=1pt]
      \begin{axis}
        [
        boxplot/draw direction=y,
        ymin=0,ymax=1,
        % ylabel={F1 Score},
        xtick={1,2,3,4},
        xticklabels={\textit{FlexRL}, \textit{Exchanger}, \textit{BRL}, Simplistic},
        cycle list={{black},{black},{black},{black}}
        ]
        \addplot+[mark = o,
        boxplot prepared={
          lower whisker  =0.1086957,
          lower quartile =0.2457298,
          median         =0.2826855,
          upper quartile =0.4511318,
          upper whisker  =0.7500000
        },
        ] coordinates {(0,0.268041237113402)(0,0.75)(0,0.24685534591195)(0,0.251968503937008)(0,0.174887892376682)(0,0.463414634146341)(0,0.521472392638037)(0,0.244604316546763)(0,0.282238442822384)(0,0.325949367088608)(0,0.438848920863309)(0,0.261213720316623)(0,0.388489208633094)(0,0.711864406779661)(0,0.140485312899106)(0,0.144086021505376)(0,0.631067961165049)(0,0.373563218390805)(0,0.108695652173913)(0,0.283132530120482)};
        \addplot+[mark = o,
        boxplot prepared={
          lower whisker  =0.2537634,
          lower quartile =0.3095743,
          median         =0.3558077,
          upper quartile =0.4015231,
          upper whisker  =0.4573171
        },
        ] coordinates {(0,0.280927835051546)(0,0.541666666666667)(0,0.35062893081761)(0,0.291338582677165)(0,0.360986547085202)(0,0.457317073170732)(0,0.429447852760736)(0,0.311750599520384)(0,0.35036496350365)(0,0.414556962025316)(0,0.384892086330935)(0,0.369393139841689)(0,0.388489208633094)(0,0.576271186440678)(0,0.307397959183673)(0,0.253763440860215)(0,0.378640776699029)(0,0.327586206896552)(0,0.292270531400966)(0,0.322289156626506)};        
        \addplot+[mark = o,
        boxplot prepared={
          lower whisker  =0.04106280,
          lower quartile =0.09632384,
          median         =0.23465516,
          upper quartile =0.40699467,
          upper whisker  =0.83333333
        },
        ] coordinates {(0,0.118556701030928)(0,0.833333333333333)(0,0.0566037735849057)(0,0.228346456692913)(0,0.0919282511210762)(0,0.463414634146341)(0,0.466257668711656)(0,0.100719424460432)(0,0.192214111922141)(0,0.325949367088608)(0,0.338129496402878)(0,0.174142480211082)(0,0.316546762589928)(0,0.635593220338983)(0,0.0816326530612245)(0,0.0838709677419355)(0,0.640776699029126)(0,0.350574712643678)(0,0.0410628019323672)(0,0.240963855421687)};
        \addplot+[mark = o,
        boxplot prepared={
          lower whisker  =0.5978495,
          lower quartile =0.6424742,
          median         =0.6642686,
          upper quartile =0.7086147,
          upper whisker  =0.7661871
        },
        ] coordinates {(0,0.608247422680412)(0,0.75)(0,0.650943396226415)(0,0.614173228346457)(0,0.683856502242152)(0,0.652439024390244)(0,0.644171779141104)(0,0.697841726618705)(0,0.737226277372263)(0,0.667721518987342)(0,0.766187050359712)(0,0.627968337730871)(0,0.661870503597122)(0,0.694915254237288)(0,0.719387755102041)(0,0.597849462365591)(0,0.640776699029126)(0,0.666666666666667)(0,0.661835748792271)(0,0.75)};
      \end{axis}
      % \node[above,font=\bfseries] at (current bounding box.north) {F1 Score};
      \end{tikzpicture}

==> Tables/suppl_tab_RLData500_Results.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{ccccccc}
      \hline
      \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
      \multicolumn{1}{c}{\textbf{Methods}} & \multicolumn{2}{c}{\textbf{Linked Records}} & \multirow{2}{*}{\textbf{FN}} & \multirow{2}{*}{\textbf{F1-Score}} & \multirow{2}{*}{\textbf{FDR}} & \multirow{2}{*}{\textbf{Sensitivity}} \\
      \cline{2-3}
      \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
      \multicolumn{1}{c}{} & \textbf{TP} & \textbf{FP} & & & &  \\
      \hline
      \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
      \textbf{\textit{FlexRL} with soundex} & $44$ & $0$ & $6$ & $.94$ & $0$ & $.88$ \\
      \textbf{\textit{FlexRL}} & $38$ & $0$ & $12$ & $.86$ & $0$ & $.76$ \\
      \textbf{\textit{Exchanger}} & $49$ & $0$ & $1$ & $.99$ & $0$ & $.98$ \\
      \textbf{\textit{BRL}} & $50$ & $1$ & $0$ & $.99$ & $.02$ & $1$ \\
      \textbf{Simplistic approach with soundex} & $20$ & $0$ & $30$ & $.57$ & $0$ & $.40$ \\
      \textbf{Simplistic approach} & $0$ & $0$ & $50$ & & & \\
      \hline
      \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
    \end{tabular}
    \caption{Performance of the compared methods on the RLData500 data with 50 links.}
    \label{tab_RLdata500_results}
\end{table}

==> Tables/suppl_tab_RLData500_Story.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{ccccccc}
        \hline
        \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
        \multicolumn{2}{c}{\textbf{Registrations}} & \textbf{First name} & \textbf{Family name} & \textbf{Birth year} & \textbf{Birth month} & \textbf{Birth day} \\
        \hline
        \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
        \multirow{3}{*}{\textbf{Data}} & \textbf{Unique} & $146$ & $108$ & $86$ & $12$ & $31$ \\
        & \textbf{Unique in encoded} & $114$ & $85$ &  &  &  \\
        & \textbf{Type} & character & character & numeric & numeric & numeric \\
        \cline{2-2}
        \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
        \multirow{2}{*}{\textbf{True Links}} & \textbf{Agree} & $.68$ & $.68$ & $.84$ & $.92$ & $.80$ \\
        & \textbf{Agree in encoded} & $.92$ & $.88$ &  &  &  \\
        \hline
        \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
    \end{tabular}
    \caption{Summary of the RLData500 data. Characteristics of the PIVs in their original format and with soundex encoding for names. Level of agreements among the 50 links referring to the same individuals. No missing value in the dataset.}
    \label{tab_RLdata500_story}
\end{table}

==> Tables/suppl_tab_SHIW_complete_results.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{ccccccc}
      \hline
      \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
      \multicolumn{1}{c}{\textbf{Methods}} & \multicolumn{2}{c}{\textbf{Linked Records}} & \multirow{2}{*}{\textbf{FN}} & \multirow{2}{*}{\textbf{F1-Score}} & \multirow{2}{*}{\textbf{FDR}} & \multirow{2}{*}{\textbf{Sensitivity}} \\
      \cline{2-3}
      \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
      \multicolumn{1}{c}{} & \textbf{TP} & \textbf{FP} & & & & \\
      \hline
      \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
      \textbf{\textit{FlexRL} (0.5)} & $2435$ & $6711$ & $3995$ & $.31$ & $.73$ & $.38$ \\
      \textbf{Simplistic approach} & $4318$ & $13807$ & $2112$ & $.35$ & $.76$ & $.67$\\
      \hline
      \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
      \textbf{\textit{FlexRL} (0.6)} & $2266$ & $5438$ & $4164$ & $.32$ & $.71$ & $.35$\\
      \textbf{\textit{FlexRL} (0.7)} & $2091$ & $4490$ & $4339$ & $.32$ & $.68$ & $.33$\\
      \textbf{\textit{FlexRL} (0.8)} & $1941$ & $3749$ & $4489$ & $.32$ & $.66$ & $.30$\\
      \textbf{\textit{FlexRL} (0.9)} & $1788$ & $3080$ & $4642$ & $.32$ & $.63$ & $.28$\\
      \hline
      \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
    \end{tabular}
    \caption{Performance of FlexRL on the complete SHIW data for several linkage probability threshold (superior to 0.5 to ensure a one-to-one assignment) and of the simplistic approach.}
    \label{tab_SHIWFull_results}
\end{table}


==> Tables/suppl_tab_SHIW_description.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{cccccccc}
        \hline
        \multicolumn{2}{c}{\textbf{Registrations}} & \textbf{Sex} & \textbf{Birth year} & \textbf{Marital status} & \textbf{Regional code} & \textbf{Birth region} & \textbf{Education} \\
        \hline
        \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
        \multirow{2}{*}{\textbf{Data}} & \textbf{Unique} & $2$ & $97$ & $4$ & $20$ & $20$ & $6$  \\
        & \textbf{Type} & categorical & categorical & categorical & categorical & categorical & categorical \\
        \cline{2-2}
        \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
        \multirow{1}{*}{\textbf{True Links}} & \textbf{Agree} & $1$ & $.98$ & $.94$ & $1$ & $.94$ & $.77$ \\
        \hline
        \noalign{\vskip\doublerulesep \vskip-\arrayrulewidth}
    \end{tabular}
    \caption{Summary of the full SHIW data of 2016 and 2020. Characteristics of the PIVs and level of agreement among the 6 430 links referring to the same individuals. There are $5\%$ of missing value in birth region in both data sets.}
    \label{tab_SHIW_Story}
\end{table}
